A Domain-Extensible Compiler with Controllable Automation of Optimisations

In high performance domains like image processing, physics simulation or machine learning, program performance is critical. Programmers called performance engineers are responsible for the challenging task of optimising programs. Two major challenges prevent modern compilers targeting heterogeneous architectures from reliably automating optimisation. First, domain-specific compilers such as Halide for image processing and TVM for machine learning are difficult to extend with the new optimisations required by new algorithms and hardware. Second, automatic optimisation is often unable to achieve the required performance, and performance engineers often fall back to painstaking manual optimisation. This thesis shows the potential of the Shine compiler to achieve domain-extensibility, controllable automation, and generate high performance code. Domain-extensibility facilitates adapting compilers to new algorithms and hardware. Controllable automation enables performance engineers to gradually take control of the optimisation process. The first research contribution is to add 3 code generation features to Shine, namely: synchronisation barrier insertion, kernel execution, and storage folding. The second research contribution is to demonstrate how extensibility and controllability are exploited to optimise a standard image processing pipeline for corner detection. The final research contribution is to introduce sketch-guided equality saturation, a semi-automated technique that allows performance engineers to guide program rewriting by specifying rewrite goals as sketches: program patterns that leave details unspecified.

==> 2-Background/backup.tex <==
\section{Overview of \Lift{}}

\includegraphics[width=\linewidth]{media/lift-compilation-steps}

\paragraph{Functional High-Level} % \Lift{} Expression}
A program is expressed in a functional language with parallel \emph{primitives} such as the ones shown in \cref{fig:primitives}.
Primitives are higher-order functions that can depend on natural numbers ($\nat$) and data types ($\data$).
For example, the dot product is written as expression (\ref{dot-high-level}).
The expression depends on a natural number $n$ and abstracts over the arrays $a$ and $b$ of $n$ floats.
$f \then g = \lambda x. g~(f~x)$ first applies the function $f$, then the function $g$.
\begin{equation}\label{dot-high-level}
\Lambda (n : nat).~\lambda (a~b : n.float).~\zip~a~b \then \map~\mulT \then \reduce~+~0
\end{equation}

\begin{figure}[ht]
{\small \begin{displaymath}\begin{array}{lll}
\map &:& (n: \nat) \to (s~t: \data) \to (s \to t) \to n.s \to n.t \\
\reduce &:& (n: \nat) \to (s~t: \data) \to (s \to t \to t) \to t \to n.s \to t \\
\prim{split} &:& (n~m: \nat) \to (t: \data) \to nm.t \to m.n.t \\
\join &:& (n~m: \nat) \to (t: \data) \to n.m.t \to nm.t \\
\transpose &:& (n~m: \nat) \to n.m.t \to m.n.t \\
\pad &:& (n~l~r: \nat) \to (t: \data) \to t \to n.t \to (l+n+r).t \\
\slide &:& (n~sz~sp: \nat) \to (t: \data) \to (sp \times n + sz - sp).t \to n.sz.t \\
\zip &:& (n: \nat) \to (s~t: \data) \to n.s \to n.t \to n.(s \times t) \\
\fst &:& (s~t: \data) \to (s \times t) \to s \\
\snd &:& (s~t: \data) \to (s \times t) \to t \\
\end{array}\end{displaymath}}
\vspace{-1em}
\caption{\Lift{} high-level primitives and their type}
\label{fig:primitives}
\end{figure}

\paragraph{Rewriting to Functional Low-Level}
Semantics-preserving \emph{rewrite rules} are applied, encoding decisions such as map fusion: $\map~f \then \map~g \to \map~(f \then g)$.
This rule states that applying $f$ over the elements of an array and then applying $g$ over the elements of the result is equivalent to applying $f$ and then $g$ over the elements of an array using a single $\map$.

Rewriting leads to a low-level functional expression where all implementation decisions are explicitly encoded.
Applying the rewrite rule (\ref{specialise-reduce-seq}) to expression (\ref{dot-high-level}) introduces the $\reduceSeq$ low-level primitive, resulting in expression (\ref{dot-seq-low-level}).
Low-level primitives indicate a specific implementation decision, and $\reduceSeq$ implements $\reduce$ with a sequential loop.
All implementation decisions are encoded in the low-level expression (\ref{dot-seq-low-level}).
This is the case because the remaining $\zip$ and $\map$ that do not indicate a particular implementation strategy will be fused into the input of $\reduceSeq$.

\begin{equation}\label{specialise-reduce-seq}
\reduce \to \reduceSeq
\end{equation}

%%% WHY HAVE ALL DECISIONS BEEN MADE HERE? EXPLAIN FUSED
\begin{equation}\label{dot-seq-low-level}
\Lambda (n : nat).~\lambda (a~b : n.float).~ \zip~a~b \then \map~\mulT \then \reduceSeq~+~0
\end{equation}

\paragraph{Translation to Imperative Low-Level}
Using a formal translation~\cite{dpia-2017} that is part of an ongoing \Lift{} design improvement, low-level expressions are translated to an imperative low-level language. The low-level expression (\ref{dot-seq-low-level}) is translated into the imperative expression shown in \cref{dot-seq-imperative}.

\begin{imperative-dpia}[label=dot-seq-imperative, caption={Imperative Low-Level expression of the dot product implementation}]
new float ($\lambda$acc. // allocate the reduction accumulator
  acc.wr := 0; // initialise the accumulator
  for n ($\lambda$i. // reduction loop
    // accumulate: zip and map are fused into the input
    acc.wr := (a@i * b@i) + acc.rd);
  output@0 := acc.rd) // output the result
\end{imperative-dpia}

\paragraph{Code Generation}
Finally, code such as C or OpenCL is generated from imperative expressions.
The generated function signature contains an output parameter followed by input parameters.
The C code shown in \cref{dot-seq-c-code} is generated from \cref{dot-seq-imperative}, and implements the dot product with a sequential reduction loop as expected.

\begin{c-code}[label=dot-seq-c-code, caption={Generated C code implementing the dot product}]
void dot(float* output, int n, float* a, float* b) {
  float acc;
  acc = 0.0f;
  for (int i = 0; i < n; i++) {
    acc = (a[i] * b[i]) + acc;
  }
  output[0] = acc;
}
\end{c-code}


\subsection{Equality Saturation}

The idea of equality saturation, introduced in \cite{tate2009-equality-saturation} and modernised in \cite{willsey2021-egg}, is to optimise programs by efficiently reasoning about many equivalent programs.
An e-graph data structure is used to efficiently encode an exponential set of equivalent programs through structural sharing.
The e-graph may become saturated if no more equalities can be added.
After reaching saturation or some other stopping criteria, the final optimised program can be selected from the equivalent programs.

~\\
Equality saturation has two big advantages that make it a promising backbone for more declarative optimisation strategies:
\begin{itemize}
   \item Rewrite order does not matter anymore since all orderings are explored in parallel
   \item Heuristics can be global and do not have to account for future transformations
\end{itemize}

\subsection{Auto-tuning}
ATLAS FFTW OpenTuner ATF

Need to give all available choices, slow, not specialised

==> 3-ImperativeCode/tuning-parameters.tex <==
\section{Introducing Tuning Parameters}
\label{sec:tuning-params}

Previous work on \Lift{} mentions that, after rewriting an expression into a low-level one, certain numerical parameters remain to be picked such as local/global thread counts, vector sizes or tile sizes \cite{lift-rewrite-2015,lift-performance-portability-2016, lift-stencil-2018}.
This is a standard auto-tuning problem that many mature frameworks aim to solve, such as the ATF auto-tuning framework \cite{rasch2017-atf} used in \cite{lift-stencil-2018}.\todo{make sure it is discussed in background}
However, work preceding this thesis provides no clear explanation as to how tuning parameters are introduced in expressions, or how the validity of parameter values is reasoned about.

\todo{so, is this section really novel / interesting?}
More recent \Lift{} work addresses the problem of finding valid combinations of parameter values \cite{mogers2020-convolution}.
Constraints are automatically inferred by traversing the expression and collecting conditions that must hold true for the parameter values to be valid.
"Parameter inference"

different constraint inference for split/asVector/slide, we have single constraint for \inlineRise{/^} operator.

A mechanism for rewrite rules to introduce tuning parameters.

Previous \Lift{} work.

\subsection{Tuning Parameters as Free Variables}

\begin{elevate-rise}
rule splitJoin(n: nat) = map f
                      $\rewritesTo$ split n $\then$ map (map f) $\then$ join
\end{elevate-rise}
\begin{elevate-rise}
rule tunedSplitJoin = map f
                   $\rewritesTo$ *tune* (n: nat). split n $\then$ map (map f) $\then$ join
\end{elevate-rise}

% def slideVectors(n: Nat): ToBeTyped[Expr] =
  % slide(n)(1) >> join >> asVector(n)
\begin{rise}
*tune* (ls0: nat) in RangeMul(1, 1024, 2). (
*tune* (ls1: nat) in RangeMul(1, 1024, 2). (
*tune* (gs0: nat) in RangeMul(1, 1024, 2). (
*tune* (gs1: nat) in RangeMul(1, 1024, 2). (
*tune* (vec: nat). (
*tune* (tile: nat) in RangeAdd(4, 1024, 1). (
$\Lambda$(n : nat) in RangeAdd(1, PosInf, vec). (
$\lambda$weights : 3.f32. (
$\lambda$input : (n + 2).f32. (
  oclRun(LocalSize(ls0, ls1), GlobalSize(gs0, gs1)) (
    input $\then$ slide (tile + 2) tile $\then$ (mapWorkGroup(0) (
      slideVectors vec $\then$ slide 3 vec $\then$
      mapLocal(0) (weightsSeqVecUnroll weights) $\then$
      asScalar
    ))) $\then$ join
)))))))))
\end{rise}

Optional Range

\paragraph{Parameter Collection}
Requires identifying tuning parameters : is free var tuned? (flag or name convention)
val parameters = collectParameters(e)
simple expression traversal

\begin{lstlisting}
ls1 in RangeMul(1,1024,2)
gs0 in RangeMul(1,1024,2)
vec in RangeUnknown
ls0 in RangeMul(1,1024,2)
gs1 in RangeMul(1,1024,2)
tile in RangeAdd(4,1024,1)
\end{lstlisting}

\paragraph{Type Inference}
Preserve (cannot be substituted)
// should we allow tuning params to be substituted during type inference?
// this could allow to restrict the search space at compile time


\paragraph{Constraint Collection}

\begin{lstlisting}
1 in RangeAdd(0,PosInf,1)
gs1 in RangeAdd(0,PosInf,ls1)
n in RangeAdd(0,PosInf,tile)
gs0 in RangeAdd(0,PosInf,ls0)
3 + tile - vec >= 1
tile /^ vec >= 1
ls1 >= 1
gs1 >= 1
n /^ tile >= 1
vec*(3 + tile - vec) >= 1
ls0 >= 1
vec >= 1
n >= 1
tile in RangeAdd(0,PosInf,vec)
vec in RangeMul(2,16,2)
gs0 >= 1
\end{lstlisting}

val constraints = collectConstraints(e, parameters)
PredicateConstraint
RangeConstraint (RangeAdd, RangeMul)

collect input nats

\begin{lstlisting}

  def collectConstraints(e: Expr, parameters: Parameters): Set[Constraint] = {
    import arithexpr.arithmetic._
    import BoolExpr._

    val paramOrInput = (parameters ++ collectInputNats(e)).map(_.name)
    val cs = collection.mutable.Set[Constraint]()

    def addPredicate(p: ArithPredicate): Unit = {
      if (!p.evaluate.contains(true)) {
        cs += PredicateConstraint(p)
      }
    }

    traverse.traverse(e, new traverse.PureTraversal {
      override def expr: Expr => monads.Pure[Expr] = { e =>
        e match {
          case DepApp(NatKind, DepApp(NatKind, DepApp(NatKind,
          DepApp(NatKind, DepApp(NatKind, DepApp(NatKind,
          rise.openCL.primitives.oclRunPrimitive(),
          ls0: Nat), ls1: Nat), ls2: Nat),
          gs0: Nat), gs1: Nat), gs2: Nat)
          =>
            for (s <- Seq(ls0, ls1, ls2, gs0, gs1, gs2)) {
              addPredicate(ArithPredicate(s, 1, ArithPredicate.Operator.>=))
            }
            for ((ls, gs) <- Seq((ls0, gs0), (ls1, gs1), (ls2, gs2))) {
              cs += RangeConstraint(gs, RangeAdd(0, PosInf, ls))
            }
          case _ =>
        }
        super.expr(e)
      }

      override def datatype: DataType => monads.Pure[DataType] = { t =>
        t match {
          case ArrayType(n, _) if n.varList.forall(v => paramOrInput(v.name)) =>
            addPredicate(ArithPredicate(n, 1, ArithPredicate.Operator.>=))
          case VectorType(n, _) if n.varList.forall(v => paramOrInput(v.name)) =>
            cs += RangeConstraint(n, RangeMul(2, 16, 2))
          case _ =>
        }
        super.datatype(t)
      }

      override def nat: Nat => monads.Pure[Nat] = n =>
        return_(n.visitAndRebuild { m =>
          if (m.varList.forall(v => paramOrInput(v.name))) { m match {
            case Prod(parts) =>
              var (num, denum) = parts.partition {
                case Pow(_, Cst(-1)) => false
                case _ => true
              }
              denum = denum.map { case Pow(b, Cst(-1)) => b }
              if (denum.nonEmpty) { // num /^ denum
                val aNum = num.fold(1: ArithExpr)(_ * _)
                val aDenum = denum.fold(1: ArithExpr)(_ * _)
                if (aNum % aDenum != Cst(0)) {
                  cs += RangeConstraint(aNum, RangeAdd(0, PosInf, aDenum))
                }
              }
            case Mod(x, _) =>
              addPredicate(ArithPredicate(x, 0, ArithPredicate.Operator.>=))
            case _ => ()
          }}
          m
        })
    })

    cs.toSet
  }
\end{lstlisting}

\paragraph{Constraint Checking}
checkConstraints
\begin{lstlisting}
sealed trait Constraint {
  def substitute(map: Map[ArithExpr, ArithExpr]): Constraint = this match {
    case PredicateConstraint(n) =>
      PredicateConstraint(n.substitute(map).getOrElse(n))
    case RangeConstraint(n, r) =>
      RangeConstraint(n.substitute(map).getOrElse(n), r.substitute(map).getOrElse(r))
  }
\end{lstlisting}
\begin{lstlisting}
  def isSatisfied(): Boolean = this match {
    case PredicateConstraint(n: ArithPredicate) =>
      n.evaluate.contains(true)
    // TODO: it feels like checking if a nat is inside a range should be part of arithexpr
    case RangeConstraint(n, RangeAdd(start, stop, step)) =>
      ArithPredicate(start, n.min, ArithPredicate.Operator.<=).evaluate.contains(true) &&
        ArithPredicate(n.max, stop, ArithPredicate.Operator.<=).evaluate.contains(true) &&
        n % step == (0: Nat)
    case RangeConstraint(n, RangeMul(start, stop, mul)) =>
      ArithPredicate(start, n.min, ArithPredicate.Operator.<=).evaluate.contains(true) &&
        ArithPredicate(n.max, stop, ArithPredicate.Operator.<=).evaluate.contains(true) &&
        isPowerOf(n.eval, mul.eval)
    case _ =>
      throw new Exception(s"no support for checking $this")
  }
}
\end{lstlisting}

1. analyse low-level Rise program to collect parameters and constraints
2. generate hypermapper configuration JSON
3. generate or use generic hypermapper Python routine
4. generate or use generic (runtime reflection with 'eval') Java executable .jar (use `sbt assembly`)
    - first use Java executor to benchmark
    - later we can use host code generation instead

contiguous memory constraint
memory alignment constraint
expression-specific constraint (tileShiftInwards)

\paragraph{Parameter Injection}
substitution

\subsection{Limitations}

\subsection{Summary}

==> 4-ImageProcessing/binomial-backup.tex <==

\section{Extending \Lift{} with Image Processing Optimisations}
\label{extension}

\Lift{} is designed to be extensible in various ways.
Implementation choices are extended by adding with rewrite rules.
Language constructs are extended by adding functional and imperative primitives.

\paragraph{Extending \Lift{} with rewrite rules}
Adding a rewrite rule allows to encode a new implementation choice.
During the rewrite process, the rule can be applied, or not.
For example, the 2D binomial filter is decomposable into two 1D filters.
This decomposition is a domain-specific transformation often used as an optimisation method.
I added the domain-specific rule (\ref{separate-dot}) to encode that the binomial filter is decomposable into a vertical filter followed by a horizontal filter.
Another rule might encode that, alternatively, the binomial filter can also be decomposed in a horizontal filter followed by a vertical filter.
Other filters are decomposable in this fashion, this rule is currently specific to the binomial filter but can be generalised.

% {\small \begin{equation}\label{separate-dot}
% \lambda nbh.~\dot~\left(\join~\weights\right)~(\join~nbh) \to \transpose \then \map~\left(\dot~\weightsh\right) \then \dot~\weightsh
% \end{equation}}

\paragraph{Extending \Lift{} with functional primitives}
Functional primitives are the basic components of \Lift{} expressions.
Adding a functional primitive allows to encode a new pattern that can be high-level (algorithmic pattern) or low-level (implementation pattern).
A new primitive most likely comes with new rewrite rules to introduce the primitive or to transform it into other primitives.
If the primitive appears in low-level expressions, translation of the primitive into the imperative language needs to be described.
% For example, the $\slide$ primitive introduced in~\cite{lift-stencil-2018} encodes the sliding window algorithmic pattern.
% I added a $\slideSeq$ primitive to encode an implementation pattern which exploits the reuse opportunity incurred by the spatial and temporal locality when sliding sequentially.
% $\slideSeq$ has the same type as $\slide$, but a different translation to imperative language.
% I also added the rule (\ref{to-slide-seq}) to encode that $\slide$ can be rewritten into $\slideSeq$.
% Two variants of this primitive can be used to either use a circular buffer or a set of rotating registers.

% {\small \begin{equation}\label{slide-seq}
%     \slideSeq: (n~sz~sp: nat) \to (\delta: data) \to (sp \times n + sz - sp).\delta \to n.sz.\delta
% \end{equation}}
% {\small \begin{equation}\label{to-slide-seq}
%     \slide \to \slideSeq
% \end{equation}}

\paragraph{Extending \Lift{} with imperative primitives}
Adding an imperative primitive allows to encode a new pattern in the low-level imperative language.
Code generation needs to be described for new imperative primitives.
% To exploit the reuse opportunity of $\slideSeq$ by rotating a set of registers, I added a \iprim{newRegRot} imperative primitive allowing to create registers and to rotate them.
% The translation of $\slideSeq$ into low-level imperative language uses \iprim{newRegRot} as shown in \cref{lst:slide-seq-imperative} for a sliding window of 3 floating point numbers.
The translation produces a prologue to initialise the registers (l.\ref{slide-seq-prologue}) followed by a steady-state loop (l.\ref{slide-seq-steady-state}).
In the steady state, the next input value is loaded (l.\ref{slide-seq-steady-input}) before using the current window for computation (l.\ref{slide-seq-steady-output}) and rotating the registers (l.\ref{slide-seq-steady-rotate}).
I also described how to generate C code for \inlineDPIA{newRegRot}, which allows to generate C code for \cref{lst:slide-seq-imperative}.

\begin{DPIA}[escapechar=|, label={lst:slide-seq-imperative}, caption={slideSeq translation to imperative IR}]
newRegRot 3 float ($\lambda$regs rotate. |\label{slide-seq-new-reg-rot}|
 for 2 ($\lambda$x. regs.wr @x := input @x); |\label{slide-seq-prologue}|
 for (size - 2) ($\lambda$x. |\label{slide-seq-steady-state}|
  regs.wr @2 := input @(x+2); |\label{slide-seq-steady-input}|
  output @y @x := f(regs.rd); |\label{slide-seq-steady-output}|
  rotate)) |\label{slide-seq-steady-rotate}|
\end{DPIA}

% \section{Rewriting the Binomial Filter}
% \label{rewrite}

% The binomial filter is expressed as the high-level \Lift{} expression (\ref{binom-high-level}).
% The first line of the expression creates a 3$\times$3 sliding window using the 1-dimensional.% $\slide$ primitive.
% The second line computes the result for every pixel by flattening the 3$\times$3 neighbourhood and the filter weights to one dimension before applying the dot product.
% % defined as $\lambda a~b.~ \zip~a~b \then \map~\mulT \then \reduce~+~0$.
% The \emph{register rotation and reduction} optimisation described in \cite{hlt-lacassagne-2014} is applied on expression (\ref{binom-high-level}) through a rewriting sequence.

% % {\small \begin{equation}\label{binom-high-level}
% % \begin{split}
% % &\map~(\slide~3~1) \then \slide~3~1 \then \map~\transpose \then \\
% % &\quad \map~(\map~(\lambda nbh.~\dot~\left(\join~\weights\right)~(\join~nbh)))
% % \end{split}
% % \end{equation}}

% To decompose the binomial filter into two 1D filters, rule (\ref{separate-dot}) is applied on expression (\ref{binom-high-level}), resulting in expression (\ref{binom-dot-separated}) where the modified sub-expression is underlined.

% % {\small \begin{equation}\label{binom-dot-separated}
% % \begin{split}
% % &\map~(\slide~3~1) \then \slide~3~1 \then \map~\transpose \then \\
% % &\quad \map~(\map~(\highlight{\transpose \then \map~\left(\dot~\weightsh\right) \then \dot~\weightsh}))
% % \end{split}
% % \end{equation}}

% A sequence of generic reorganisation rules (detailed in \cref{binom-reorganise}) is applied to rewrite expression (\ref{binom-dot-separated}) into expression (\ref{binom-reorganised}).

% % {\small \begin{equation}\label{binom-reorganised}
% % \slide~3~1 \then \map~(\transpose \then \map~(\dot~..) \then \slide~3~1 \then \map~(\dot~..))
% % \end{equation}}

% Expression (\ref{binom-reorganised}) is finally rewritten into expression (\ref{binom-low-level}) by selecting low-level primitives where appropriate using rewrite rules.

% % {\small \begin{equation}\label{binom-low-level}
% % \slide~3~1 \then \highlight{\mapSeq}~(\transpose \then \map~(\highlight{\dotSeq}~..) \then \highlight{\slideSeq}~3~1 \then \map~(\highlight{\dotSeq}~..))
% % \end{equation}}

% Expression (\ref{binom-low-level}) corresponds to an implementation using the \emph{register rotation and reduction} optimisation described in \cite{hlt-lacassagne-2014}.
% The code generated for expression (\ref{binom-low-level}) is shown in \cref{lst:binom-c-code}.
% As can be observed, the vertical part of the decomposed binomial filter is computed and stored in 3 registers that are used to compute the horizontal part of the filter and rotated as needed.
% % The outer $\mapSeq$ generates the outer loop on lines (l.\ref{binom-c-line-loop}), while the $\slideSeq$ generates the inner prologue (l.\ref{binom-c-column-prologue}) and steady-state (l.\ref{binom-c-column-loop}) loops on columns.

% \begin{c-code}[escapechar=|, label={lst:binom-c-code}, caption={Generated C code}]
% void blur(float* output, int h, int w, float* input) {
%   for (int y = 0; y < (h-2); y = (1 + y)) { |\label{binom-c-line-loop}|
%     float regs[3];
%     for (int x = 0; x < 2; x = (1 + x)) { ... }  |\label{binom-c-column-prologue}|
%     for (int x = 0; x < (w-2); x = (1 + x)) {  |\label{binom-c-column-loop}|
%       float acc_v = 0.0f;
%       acc_v += 0.25f * input[(2+x+(y*w) + (0*w))];
%       acc_v += 0.50f * input[(2+x+(y*w) + (1*w))];
%       acc_v += 0.25f * input[(2+x+(y*w) + (2*w))];
%       regs[2] = acc_v;
%       float acc_h = 0.0f;
%       acc_h += 0.25f * regs[0];
%       acc_h += 0.50f * regs[1];
%       acc_h += 0.25f * regs[2];
%       output[(x + (-2 * y) + (y * w))] = acc_h;
%       regs[0] = regs[1];
%       regs[1] = regs[2]; }}}
% \end{c-code}

% \section{Translation Modification}
% \label{translation}

% % In fact, the original \Lift{} translation to imperative and code generation could not generate code for the sub-expression (\ref{slide-fusion-target}), because the formalism did not explain how to fuse the two $\map$s in the $\slideSeq$ loop.

% % {\small \begin{equation} \label{slide-fusion-target}
% % \map~(\dotSeq~..) \then \slideSeq~3~1 \then \map~(\dotSeq~..)
% % \end{equation}}

% I identified three possible solutions to generate code for expression (\ref{slide-fusion-target}):
% \begin{enumerate}
%     \item % Each $\map$ can be rewritten into a $\mapSeq$ as in expression (\ref{slide-no-fusion}).
%     However this is not expressing the desired implementation because there are now two additional sequential loops that will also generate unwanted temporary results.
%     This solution is clearly not suitable.

%     % {\small \begin{equation} \label{slide-no-fusion}
%     % \mapSeq~(\dotSeq~..) \then \slideSeq~3~1 \then \mapSeq~(\dotSeq~..)
%     % \end{equation}}

%     % \item The $\slideSeq$ primitive can be modified to take two additional arguments, a function to apply on its input and another to apply on its output.
%     % In this case, the desired code can be generated by rewriting expression (\ref{slide-fusion-target}) (where $\slideSeq$ would additionally take two identity functions as parameters) into expression (\ref{slide-primitive-fusion}) with the addition and application of the two rewrite rules (\ref{slide-primitive-input-fusion}) and (\ref{slide-primitive-output-fusion}).

%     % {\small \begin{equation} \label{slide-primitive-fusion}
%     % \slideSeq~3~1~(\dotSeq~..)~(\dotSeq~..)
%     % \end{equation}}
%     % {\small \begin{equation} \label{slide-primitive-input-fusion}
%     % \map~f \then \slideSeq~n~m~g~h \to \slideSeq~n~m~(f \then g)~h
%     % \end{equation}}
%     % {\small \begin{equation} \label{slide-primitive-output-fusion}
%     % \slideSeq~n~m~f~g \then \map~h \to \slideSeq~n~m~f~(g \then h)
%     % \end{equation}}
    
%     \item Finally, the formal translation to imperative language can be modified to directly explain how code is generated for expression (\ref{slide-fusion-target}).
% \end{enumerate}

% %I decided to use the third solution because it defines a reusable fusion mechanism and allows the low-level $\slideSeq$ primitive to keep the same type as the high-level $\slide$ primitive.
% Modifying the core \Lift{} compiler required me a significant amount of work and reflection.
% This change is not an extension, but it is an incremental improvement to the common framework that is neither domain-specific nor hardware-specific, and should benefit to many other expressions and use cases.

% \section{Preliminary Evaluation}
% \label{evaluation}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.6\textwidth]{media/odroid-cpu-seq-results.pdf}
%   \caption{Runtime of sequential variants (1920$\times$1080 pixels, ARM CPU, Odroid XU4)}
%   \label{fig:seq-results}
% \end{figure}

% In a preliminary evaluation, the code produced with \Lift{} expressions is compared against handwritten C code for sequential execution.
% Figure \ref{fig:seq-results} compares the runtime of 4 binomial filter variants on an ARM Cortex CPU.
% % Each variant different impletations choices and trade-offs between redundant computations and memory accesses.
% \begin{itemize}
%     \item \texttt{base} computes the result for every pixel, not storing any intermediate results.
%     \item \texttt{factorised} does the same but decomposes the filter computations.
%     With \Lift{} the rewrite rule (\ref{separate-dot}) is used.
%     \item \texttt{separated} uses an intermediate for the vertical reduction of the entire image.
% %\texttt{scanline} uses an intermediate for each line.
%     \item \texttt{rot-values} uses register rotation, only keeping a sliding window of vertical reductions in memory.
%     %With \Lift{} the $\slideSeq$ and \iprim{newRegRot} primitives are used.
% \end{itemize}

% \Lift{} achieves competitive performance compared to the handwritten code.
% The \Lift{} \texttt{rot-values} is the fastest variant overall (11.9ms, 2.5$\times$ faster than the slowest \texttt{base}).
% % , while the handwritten \texttt{rot-values} has room for improvement.

% % However, Halide obtains poor performance on \texttt{rot-indices} because it was not designed for this use-case.% and expects coarser granularity.

% \clearpage
% \section{Performance Potential}
% \label{potential}

% To investigate the performance potential of \Lift{} for parallel execution, I compared code generated with Halide against handwritten code.
% The handwritten code is written in a style that we should to be able to generate with \Lift{}.
% Figures \ref{fig:par-a15-results} and \ref{fig:par-a7-results} compare the runtime of the best binomial filter variants on ARM Cortex CPU for an image of 1920$\times$1080 pixels.
% The execution is now locked to either the big ARM Cortex-A15 cores or the little ARM Cortex-A7 cores of the Odroid XU4 to have a reliable thread placement.
% \begin{itemize}
%     \item \texttt{scanline-vec-par} uses an intermediate for the vertical reduction of each line, with vectorisation and multi-threading.
%     \item \texttt{rot-values-vec-par} adds vectorisation and multi-threading to \texttt{rot-values} as described in \cite{hlt-lacassagne-2014}.
% \end{itemize}

% \begin{figure}[hb]
%   \centering
%   \includegraphics[width=0.6\textwidth]{media/odroid-cpu-par-a15-results.pdf}
%   \caption{Runtime of parallel variants on big ARM A15 cores}
%   \label{fig:par-a15-results}
% \end{figure}
% \begin{figure}[hb]
%   \centering
%   \includegraphics[width=0.6\textwidth]{media/odroid-cpu-par-a7-results.pdf}
%   \caption{Runtime of parallel variants on little ARM A7 cores}
%   \label{fig:par-a7-results}
% \end{figure}

% The Halide algorithm and schedule is written by hand and the \texttt{scanline-vec-par} variant corresponds to the recommended schedule for a 3$\times$3 blur.
% Halide separates algorithm from schedule, but for the binomial filter the algorithm has to be modified to separate the convolution and the \texttt{rot-values-vec-par} variant cannot be expressed with the scheduling language\footnote{\url{https://github.com/halide/Halide/issues/2905\#issuecomment-382826789}}.
% The handwritten \texttt{rot-values-vec-par} is the fastest variant overall:
% \begin{itemize}[nosep]
%     \item 4.5ms on the A15s, 1.8$\times$ faster than the best Halide variant.
%     \item 13.8ms on the A7s, 1.4$\times$ faster than the best Halide variant.
% \end{itemize}

% This demonstrates that once we are able to generate \texttt{rot-values-vec-par} with \Lift{}, we will produce faster code than Halide for the binomial filter on these embedded CPUs.

% Vectorised and multi-threaded code has already been generated with \Lift{} for other applications in previous work, and generating \texttt{rot-values-vec-par}  with \Lift{} should be feasible via a few extensions. 


==> B-RewriteSteps.tex <==
\chapter{Binomial Filter Rewrite Steps}
\label{binom-reorganise}

We introduce the following notation for brevity:

{\small \begin{displaymath}\begin{array}{ll}
* &= \map \\
T &= \transpose \\
S_h &= \slide~3~1 \\
S_v &= \slide~3~1 \\
D_h &= \dot~\weightsh \\
D_v &= \dot~\weightsv \\
D_{2d} &= \lambda nbh.~\dot~\left(\join~\weights\right)~(\join~nbh) \\
\end{array}\end{displaymath}}

Using this notation, the complete rewrite sequence used for the \emph{register rotation and reduction} optimisation in \cref{rewrite} is:

{\small \begin{displaymath}\begin{array}{l|l}
\textit{Current Expression} & \textit{Applied Rule} \\
\hline
*S_h \then S_v \then *T \then **D_{2d}
& D_{2d} \to T \then *D_v \then D_h \\
*S_h \then S_v \then *T \then **(T \then *D_v \then D_h) 
& *f \then S \to S \then **f \\
S_v \then **S_h \then *T \then **(T \then *D_v \then D_h)
& *f \then *g \to *(f \then g) \\
S_v \then **S_h \then *(T \then *(T \then *D_v \then D_h))
& *f \then *g \to *(f \then g) \\
S_v \then **(S_h \then T \then *(T \then *D_v \then D_h))
& *S \then T \to T \then S \then *T \\
S_v \then *(T \then S_h \then *T \then *(T \then *D_v \then D_h))
& *f \then *g \to *(f \then g) \\
S_v \then *(T \then S_h \then *(T \then T \then *D_v \then D_h))
& T \then T \to  \\
S_v \then *(T \then S_h \then *(*D_v \then D_h))
& *(f \then g) \to *f \then *g \\
S_v \then *(T \then S_h \then **D_v \then *D_h)
& S \then **f \to *f \then S \\
S_v \then *(T \then *D_v \then S_h \then *D_h)
& \reduceSeq; \reduceSeq; \slideSeq; \mapSeq \\
\end{array}\end{displaymath}}

